Efficient stochastic simulation of rate equations and photon statistics of nanolasers

Based on a rate equation model for single-mode two-level lasers, two algorithms for stochastically simulating the dynamics and steady-state behaviour of micro- and nanolasers are described in detail. Both methods lead to steady-state photon numbers and statistics characteristic of lasers, but one of the algorithms is shown to be significantly more efficient. This algorithm, known as Gillespie's First Reaction Method (FRM), gives up to a thousandfold reduction in computation time compared to earlier algorithms, while also circumventing numerical issues regarding time-increment size and ordering of events. The FRM is used to examine intra-cavity photon distributions, and it is found that the numerical results follow the analytics exactly. Finally, the FRM is applied to a set of slightly altered rate equations, and it is shown that both the analytical and numerical results exhibit features that are typically associated with the presence of strong inter-emitter correlations in nanolasers.

==> App_Algorithms.tex <==


\section{Derivation of the FTI and FRM algorithms}\label{App:Algorithms}
In this appendix, we will give a slightly more detailed description of why the FTI and FRM algorithms have the specific forms described in the main text. We will describe in some detail the probability theoretical considerations that go into the derivation of the algorithms, though the full mathematical description is beyond the scope of this paper; see instead e.g. \cite{Gillespie1976}.

As mentioned in Sec. \ref{Sec:StochSim}, our aim is to simulate the interaction of a collection of discrete photons and emitters in a single-mode optical cavity, whose dynamics are governed by the set of rate equations \eref{RateEqs_p}-\eref{RateEqs_e}. To perform these stochastic simulations, we make a fundamental assumption common to the stochastic formulation of chemical kinetics \cite{Gillespie1976}: There exist a set of constants $c_{\mu}$ for each type of event $\mu$, which depend only on the physical properties of the system (not particle numbers), such that
    \ali{c_{\mu} dt =& \text{ Average probability, to first order in  }\nonumber \\
    & \text{ $dt$, that one particular combination of } \nonumber \\
    & \text{ photons and/or emitters  will undergo} \label{c_mu}\\
    &\text{ an event of type $\mu$ during the next } \nonumber \\
    &\text{ time increment } dt. \nonumber
    }
For instance, the probability that a particular photon in the cavity mode will be lost through the cavity mirrors during a time increment $dt$, averaged over all photons in the cavity mode, is $\gamma_{c} dt + o(dt)$, where $o(dt)$ are extra terms satisfying $o(dt)/dt \rightarrow 0$ as $dt\rightarrow 0$; In other words, $c_{c} = \gamma_{c}$. Likewise, the probability that a particular photon in the cavity mode will cause a specific excited emitter to emit in a stimulated emission event during $dt$ is $\gamma_{r} dt + o(dt)$, so $c_{st} = \gamma_{r}$. Additionally, if at time $t$ the numbers of photons and excited emitters are $n_{p}(t)$ and $n_{e}(t)$, respectively, we can define the functions $h_{\mu}$ as
    \ali{h_{\mu} =& \text{ Number of distinct combinations of photons } \nonumber \\
    & \text{ and/or emitters that can undergo an event} \label{h_mu}\\
    &\text{ of type $\mu$, given that the current particle} \nonumber \\
    &\text{ numbers are }  (n_{p}(t) , n_{e}(t)). \nonumber
    }
For instance, the number of photons which could potentially leak out of the cavity is the current photon number, i.e. $h_{c} = n_{p}(t)$; and since each of the $n_{p}(t)$ photons can prompt a stimulated emission event from each of the $n_{e}(t)$ excited emitters, we take $h_{st} = n_{e}(t) n_{p}(t)$. Combining the two quantities defined in eqs.  \eref{c_mu} and \eref{h_mu}, we can define the rates, or propensity functions, $a_{\mu}$ as
    \ali{a_{\mu} dt =& \ h_{\mu} c_{\mu} dt \nonumber \\
    =& \text{ Probability, to first order in $dt$, }\nonumber \\
    & \text{  that an event of type $\mu$ will } \label{a_mu} \\
    & \text{ occur during the next time } \nonumber\\
    &\text{ increment } dt. \nonumber
    }
In \cite{Mork2018}, the stochastic simulations are carried out by choosing a fixed time increment $dt$ and using the quantities defined above to determine how many of each type of event $\mu$ that happen at every time step: It is suggested that the total number of events of type $\mu$ happening during the time increment $dt$ follows a binomial distribution, $\text{Binom}(h_{\mu} , c_{\mu}dt)$, based on the idea that each individual event which happens can be seen as a success in a Bernoulli trial, i.e. a yes/no-experiment, whose probability of success is $c_{\mu} dt$ (Of course this assumes that $dt$ is small enough that $c_{\mu}dt\leq 1$). As an example, the number of photons lost through the cavity mirrors between $t$ and $t+dt$ is taken to be a random integer drawn from the binomial distribution $\text{Binom}(n_{p}(t) , \gamma_{c} dt)$, since the average probability of losing one photon is $\gamma_{c} dt$ and there are $n_{p}(t)$ "tries". In order to speed up the simulations, a further assumption is made in \cite{Mork2018}, namely that the time increment $dt$ may be chosen sufficiently small that the binomial distributions $\text{Binom}(h_{\mu} , c_{\mu}dt)$ may be replaced by Poisson distributions $\text{Poiss}(h_{\mu}c_{\mu} dt) = \text{Poiss}(a_{\mu} dt)$. This removes the upper bound on the integers that may be drawn, introducing the risk that e.g. the number drawn for how many photons are lost through the cavity mirrors is greater than the number of photons currently in the cavity mode, but by choosing a sufficiently small time increment $dt$, this risk is minimal.

While the replacement of binomial distributions by Poisson distributions significantly reduces computation times for the algorithm of \cite{Mork2018}, the simulation must still run for several hours to obtain satisfactory photon statistics for all pump values. Implementing a more efficient algorithm is therefore highly desirable, and to do this we can change the fundamental viewpoint in the simulation: Instead of determining how many events of each type occur during a fixed time increment, we can try to determine the length of time until \emph{some} event occurs and then determine which type of event occurs. There are several ways of doing this, but Gillespie's First Reaction Method is based on the following idea: For each $\mu$ we can find a tentative time $\tau_{\mu}$ until an event of type $\mu$ would occur, assuming no other event occurs before, and then we choose the smallest of these tentative times, $\tau_{\mu_0}$, as the time until an event actually occurs. The corresponding event type, $\mu_{0}$, is chosen as the event type that happens. To generate the random $\tau_{\mu}$'s, we should consider the probabilities at time $t$ for an event of type $\mu$ to happen between times $t+\tau$ and $t+\tau +dt$. We may compute such a probability as the product of the probability that no event of type $\mu$ happens between $t$ and $t+\tau$, given by
    \eql{ProbEventMu}{P_{0}(\tau) = \exp(- a_{\mu} \tau), }
and the probability $a_{\mu} dt$ that an event of type $\mu$ does occur during an interval of length $dt$ \cite{Gillespie1976}. In other words, the probabilities that we are looking for are of the form
    \eql{ExpDistMu}{P_{\mu}(\tau) \;dt = a_{\mu}  \exp(- a_{\mu} \tau)\;dt.}
To generate the random tentative times $\tau_{\mu}$, we can therefore draw random numbers from the distributions $P_{\mu}(\tau)$, which are essentially exponential distributions with parameters $a_{\mu}$. 

